Cross-Lingual Knowledge Transfer for Clinical Phenotyping

Clinical phenotyping enables the automatic extraction of clinical conditions from patient records, which can be beneficial to doctors and clinics worldwide. However, current state-of-the-art models are mostly applicable to clinical notes written in English. We therefore investigate cross-lingual knowledge transfer strategies to execute this task for clinics that do not use the English language and have a small amount of in-domain data available. We evaluate these strategies for a Greek and a Spanish clinic leveraging clinical notes from different clinical domains such as cardiology, oncology and the ICU. Our results reveal two strategies that outperform the state-of-the-art: Translation-based methods in combination with domain-specific encoders and cross-lingual encoders plus adapters. We find that these strategies perform especially well for classifying rare phenotypes and we advise on which method to prefer in which situation. Our results show that using multilingual data overall improves clinical phenotyping models and can compensate for data sparseness.

==> sections/Q_Figures.tex <==
\begin{figure*}[t!]
  \centering
   \includegraphics[scale=0.5]{images/Methodology_Grafik.png}
  \caption{Baseline methods}
\label{fig:methodology}
\end{figure*}

==> sections/Z_Discussion.tex <==


We experimented with knowledge transfer for all possible combinations and fine-tune order of the knowledge transfer approach.
Interestingly both datasets, although differing in term density, length .... they both perform best when incorporating knowledge from all other datasets. Surprisingly the approach of combining the datasets brings different benefits to each. For CodiEsp translating the text into English and using a domain-specific model brings best performance, while for Ahepa the method of sequential Adapter training results to the best performance slightly better than the monolingual model. (The same results can be seen in the long tail...) 


It seems that the order of the training sequence is not clear which works best.


Task, low-resource datasets monolingual works better. 
Multilingual encoders have averaged representation and requires more data see XLMR greek/spanish
Adapters are also not that good on small data. 

Explain why CodieTask is more complex than Achepa. 
Can we say sth about complexity? more samples per label!!


\paragraph{Language representation is important}

". The multilingual models tend to fragment the words more than GREEK-BERT,
especially M-BERT variants, whose fragmentation ratio is approximately twice as large. XLM-R has a lower fragmentation ratio than
M-BERT, as it has four times more sub-words covering Greek.
All three multilingual models often over-fragment Greek words.
For example, in M-BERT-UNCASED ‘κατηγορουμενος’ becomes
[‘κ’, ‘ ατ’, ‘ η΄, ‘ γο’, ‘ ρου’, ‘ μενος’], and ‘γνωμη’ becomes [‘γ’, ‘ ν’,
‘ ωμη’], but both words exist in GREEK-BERT’s vocabulary. We
suspect that, despite the ability of sub-words to effectively prevent"
Recall
that these models cover Greek with just a small portion of their
sub-word vocabularies (approx. 2\% for XLM-R a
which may cause excessive word fragmentation\todo{report fertility rates}.  
As we have seen in the Results mentioned above. The models 
XLM-R has been trained on the CC-100 corpus in 100 languages. It is important to note that there is a big imbalance between the languages. The corpora contains 55608(M) english, 9374(M) spanish and 4285(M) greek tokens with a shared vocabulary of 250K subwords and one tokenizer. Spanish belongs to the languages that are relatively well represented and Greek to the languages that are not that well represented.
\textbf{When comparing to the monolingual counterparts for both tasks to isolate the complexity of each task the performance gap between the monolingual model and the XLMR trained on a single dataset is higher for the Achepa Dataset which reflects the lower amount of training data in greek than in spanish.}
In addition the Spanish BERT uses 31K subwords . 
GreekBERT is using a vocabulary of 35k subwords. The fact, that the greek clinical notes are shorter, have a high density of medical terms and the large vocabulary of GreekBERT is decisive for a good representation as reflected in the performance of GreekBERT.  

The fact, that XLM-R has seen a big amount of Spanish data is beneficial and although english and spanish are from different language branches and have more common roots than with greek they benefit from each other in downstream tasks.






\textit{Domain-specific training performs well for the codiEsp data where data has been translated with an MT trained on biomedical text but this is not the case for Achepa where the translator has not.}

\paragraph{Adding a third language}
Even though the greek language is very different from spanish all of the transfer techniques manage to succesfully incorparate knowledge from both datasets and boost the results compared to the multilingual encoder counterparts. 






  






%In particular,
%we show that translating different parts of each
%instance separately (e.g., the premise and the hypothesis in NLI) can alter superficial %patterns in the
%data (e.g., the degree of lexical overlap between
%them), which severely affects the generalization
%ability of current models. B

==> sections/Z_Introduction.tex <==

\section{Introduction}

The importance to share medical and clinical knowledge became very apparent throughout the COVID-19 pandemic. In the past a lot of institutions and professionals were reluctant to share data due to privacy concerns \cite{sharing_is_caring}. Now, in the face of the pandemic initiatives such as \cite{multicenter_EHR_PACMED} came to life, where hospitals in the Netherlands were share pseudonymized clinical data to enable better and faster treatment for this global challenge. \todo{bridge} The prevalence of endemic diseases is restricted to certain regions or populations but may also spread to other regions with time. The Chagas disease is an example of such a case. It poses a major public health problem in Latin America and during the last years, it has become an emerging problem in North America and Europe due to increasing international migration \cite{chagas}. It is estimated that 300,000 persons with the disease live in the United States\footnote{\url{https://www.cdc.gov/parasites/chagas/epi.html)}}.
Additionally, the fact that precision medicine is becoming more important underlines the benefits of sharing clinical knowledge not only within one country but also across borders. 
English is the common language of science, and yet, although estimates vary, only around 5\% of the world's population has English as a first language, and one in five to one in 14 people are estimated to speak English as a second language \cite{health_research_languages}. The dominance of the English language in publications and research is not only encountered in the medical domain \cite{languages_of_medicine} but also NLP research focused on the English language until recently. To the contrary medical professionals use the native language spoken e.g. within hospitals to write clinical notes but also to communicate with each other and the patients. To incorporate clinical knowledge from different regions of the world Clinical decision support (CDS) systems do not only need to understand and extract relevant facts from such notes but also to learn complex relations between them across different languages.
Pre-trained monolingual language models such as BERT \cite{bert} have shown to be able to both extract information from noisy text and to capture task-specific relations in an end-to-end fashion \cite{tenney, explainbert} 

The multilingual counterparts such as XLM-R \cite{XLMR} have shown great results on multilingual benchmarks \todo{We demonstrate empirically that a large English language model coupled with modern machine translation outperforms native language models in most Scandinavian languages}
Machine Translation. Multilingual Benchmarks \cite{Xtreme_benchmark, xtreme_r}
\cite{use_machine_translation} 
 \cite{xl-translations_downstream} 


\todo{While achieving state-of-the-art results in multiple tasks and languages, translation-based cross-lingual transfer is often overlooked in favour of massively multilingual pre-trained encoders. Arguably, this is due to its main limitations: 1) translation errors percolating to the
classification phase and 2) the insufficient expressiveness of the maximum-likelihood translation. To remedy this, we propose a new technique that integrates both steps of the traditional pipeline (translation and classification) into a single model, by treating the intermediate translations as a latent random variable.}

Adapters\cite{madX} [A lot of research has been done in Clinical Decision support mainly in english yada yada yada pubmedbert and so on].  \cite{federated_learning}
data from multiple sites is complementary. 

state challenges! 
can we simply translate? 
can we use adapers?
can we use xmlr?
ist multilingualitaet eine Loesung? 

\begin{itemize}

\item{
\textbf{Why is it important to categorize patients by diagnosis?}
epidemiological data of a clinic 
patient phenotypes for disease development research 
eligibility for clinical trials 
cost estimation}

\item{\textbf{Why is it important to augment clinical data from different countries?}
globalization of diseases 
low volume of certain diseases
more effective treatments
=> multilingual Clinical Decision Support system
labels and targets are not word, 
more context 
}

\item{\textbf{Why Diagnosis and not ICD-10?}, 
- move to introdcution of data

usage of ICD-10 code assignment differs (e.g. only main diagnosis gets an ICD-10 code), due to direct impact on billing may be biased, clinically more relevant and no 1:1 relationship between Ahepa diagnosis and ICD10,
Problem with granularity and e.g. cancer and cardiopathies 
CCSR good compromise due to the generalizability}

\item{\textbf{Why only codie labels?} 
dataset public, and focus on diseases known by codie for better analysis}

\end{itemize}

Here we want to investigate the task of diagnosis prediction \todo{unknown task?} in a multilingual setting. We thus base our work on these models and pose the following questions:

\begin{itemize}

\item{\textbf{Generalizability} (How well does it transfer from clinic to clinic without having seen data)
This is relevant since different clinics do not only use different languages, but have other medical focus (ICU, broad, cardiology), style of writing and  format for the text too.}

\item{\textbf{Few-shot and Zero-shot} (long-tail, low-volume of patients (not necessarily changing frequency) e.g.  takotsubo cardiomyopathy\footnote{\url{https://en.wikipedia.org/wiki/Takotsubo_cardiomyopathy}}}

\item{\textbf{Data augmentation} works although we have different distributions and cohorts }

\item{What are differences in \textbf{translation and original language} is it better to translate and use a big pre-trained model instead of text in original language?}
 Can knowledge be complemented throughout languages?
\textbf{Effect of translation and tokenizers}

\item{ALL Labels? for best model? }

\end{itemize}

\paragraph{Contributions.} 
We summarize the major contributions of this work as follows:\\

\textbf{EHRs have been studied extensively....}\\
\textbf{CDS and introduction of phenotyping task}\\
%Clinical descision support(CDS) systems manage and process clinical data to derive connections between patients, their past medical history and clinical research to support clinical workflows \cite{cdss}. One of the fundamental tasks of such a system is \textit{Phenotyping} \cite{phenotype}. Phenotyping is the extraction of a patient medical conditions from free clinical text. This is critical for a variety of tasks that are important for clinics. Such tasks include epidemiological research studies, research on disease development and personalized treatments, monitor health trends or facilitate medical billing and reimbursement. We here study the task of automatic phenotyping in a \textit{multilingual} setting and compare different approaches as demonstrated in Figure \ref{fig:methodology}. We use contextualized encoders that have already proven to work well in many domains including the medical such as ICD-code prediction \cite{bert_medical_code_assignement} and clinical outcome prediction \cite{clinical_outcome} to predict medical conditions from clinical notes of three hospitals located in three different countries written in a different language i.e. english, spanish and greek. 
\textbf{knowledge transfer between languages and hospitals, importance of sharing data}\\
%The extraction and transfer of knowledge from different hospitals with clinical notes written in different languages has been rarely studied. The importance to share medical and clinical knowledge across clinics and countries became very apparent throughout the current COVID-19 pandemic. The dominance of the English language in publications and research is not only encountered in the medical domain \cite{languages_of_medicine} but also NLP research focused on the English language until recently. To the contrary medical professionals use the native language spoken e.g. within hospitals to write clinical notes but also to communicate with each other and the patients. 
\textbf{bridge to the use of Bert Encoders}\\
%To incorporate clinical knowledge from different regions of the world Clinical decision support (CDS) systems do not only need to understand and extract relevant facts from such notes but also to learn complex relations between them across different languages. Pre-trained monolingual language models such as BERT \cite{bert} have shown to be able to both extract information from noisy text and to capture task-specific relations in an end-to-end fashion \cite{tenney, explainbert}. Cross-domain Cross-language  + 
\textbf{importance of multilinguality}\\
%English is the common language of science, and yet, although estimates vary, only around 5\% of the world's population has English as a first language, and one in five to one in 14 people are estimated to speak English as a second language \cite{health_research_languages}. The dominance of the English language in publications and research is not only encountered in the medical domain \cite{languages_of_medicine} but also NLP research focused on the English language until recently. To the contrary medical professionals use the native language spoken e.g. within hospitals to write clinical notes but also to communicate with each other and the patients. To incorporate clinical knowledge from different regions of the world Clinical decision support (CDS) systems do not only need to understand and extract relevant facts from such notes but also to learn complex relations between them across different languages.
\textbf{covid and endemic diseases}\\
%Clinical knowledge exchange very important as e.g. in the face of a pandemic like COVID-19.
%Clinical Notes and Automating the categorization of patients will allow studies about risk and prognostic factors, personalized treatments as well as disease development, cost estimation by understanding the endemic distribution of diseases. Endemic diseases are restricted to certain regions or populations but may also spread to other regions with time. The Chagas disease is an example of such a case. It poses a major public health problem in Latin America and during the last years, it has become an emerging problem in North America and Europe due to increasing international migration \cite{chagas}. It is estimated that 300,000 persons with the disease live in the United States\footnote{\url{https://www.cdc.gov/parasites/chagas/epi.html)}}.
%Additionally, the fact that precision medicine is becoming more important underlines the benefits of sharing clinical knowledge not only within one country but also across borders. 
%Except low-resource languages the population of a country like greece is also important in %order to be able to say things about diseases that generally have a low occurence. 
%Such an example is
%\textbf{Why is it important to augment clinical data from different countries?}
%globalization of diseases 
%low volume of certain diseases e.g takotsubo myocardiopathy
%more effective treatments
%=> multilingual Clinical Decision Support system

\textbf{Main Question and challenges}\\
How can clinics with little data solve the task with clinical notes not written in english?\\
%Clinical coding requires the analysis and transformation of
%medical narratives into a structured or coded format using internationally recognized classification systems like ICD-10.
%What are the challenges in building a Clinical Decision Support system that understands multiple languages and combines data from multiple different clinical sites, given that the disease distribution is different, the focus of the each clinic, the form and style of reporting.   
%\begin{itemize}
  %  \item{different form of documenting} 
  %  \item{different writing styles (different doctors within hospital and beyond)}
 %   \item{different languages} 
  %  \item{different distribution of endemic diseases between hospitals}
   % \item{power-law distribution}
  %  \item{domain specific language}
  %  \item{real world data: stichwortartig, abbreviations ...}
  %  \item{languages belong to different branches of the same language family but especially %greek is also typologically different}
%\end{itemize}
%using different writing styles and multiple languages the explained variance is increased. 
%having diseases and symptoms appear in multiple contexts and expressed in different words.
%\textbf{Usually in cross-lingual research a cross-lingual model using task-specific data from %one language, and evaluate that task in a different language instead of using transfer learning between the datasets.}
%We consider the phenotype classification task, input, output etc.
%Figure 1 describes the setup for this paper
%The greek language has been rarely studied in this context. 
%Afaik we are the first 
%The models have to learn complex patterns between the content and context of the notes, the relation between different styles of writing and forms of documenting as well as between languages.
can we simply translate? \\
can we use multilingual encoders?\\
Is training the full network necessary or are Adapters enough?\\
What is the best solution for a low number of clinical documents in low resource languages?\\ 
when should what method be used?\\





==> sections/Z_Related_work.tex <==
\section{Related Work}


Related work sollte eine Seite sein zu den Themen die in der Introduction angesprochen werden.
\subsection{Phenotyping Task with Electronic Health Records}
\paragraph{icd coding}
\paragraph{CCSR coding}
some papers about the task

\subsection{Pre-trained Language Models for Clinical Domain}
pubmedbert, biobert and spanish biobert?

\paragraph{multilingual vs crosslingual}
\subsection{cross lingual transfer}
\cite{XLMR} is a state of the art cross-lingual model 
\subsection{multilingual and cross lingual transfer in healthcare}
brasilian model \cite{brasilian_biobert}
-\cite{schafer_multilingual_icd}  uses translated data to predict icd10 codes and learning a-priori rules.

!!!always with focus on medical topics


\textbf{Translate-test}: Fine-tune English model on an English training set and evaluate on the machine-translated test set. This imitates the scenario where you just machine-translate your data, use an English model, and hope for the best.

\textbf{Translate-train}: Machine-translate the English training set to another language and fine-tune a multilingual model on that. In this case, the test set remains in the original language.


Recently \cite{Xtreme_benchmark} to incorporate a number of previously well known tasks in English in a multilingual setting. 

\cite{xl-translations_downstream}
adapting translation to perform downstream task
\cite{zero_shot_Ponti} is this relevant?
Most combinations of NLP tasks and language varieties lack in-domain examples for
supervised training because of the paucity
of annotated data. How can neural models
make sample-efficient generalizations from
task–language combinations with available
data to low-resource ones?

\cite{opus_mt} off the shelf translation systems that are state of the art.


\cite{bert_medical_code_assignement}
Most closely related papers
\cite{use_machine_translation} we should stop using monolingual models but instead translate. 
this works well for some languages but not for others.

\cite{translationArtifacts} show that translations simplify language and may support downstream task BUT improvements can be seen due to the fact that translate test and translate train are used and not because of augmentation of data

maybe something about small-data


Related work sollte eine Seite sein zu den Themen die in der Introduction angesprochen werden.
\subsection{Phenotyping Task with Electronic Health Records}
\paragraph{icd coding}
\subsection{multilingual cross lingual tranfer}
!!!always with focus on medical topics
\subsection{Pre-trained Language Models for Clinical Domain}

\subsection{cross lingual transfer}
Cross-lingual transfer: Fine-tune multilingual model on English training set and evaluate on each language’s test set. This is, in some sense, the ultimate test of a model that truly understands multiple languages. 
Translate-test: Fine-tune English model on an English training set and evaluate on the machine-translated test set. This imitates the scenario where you just machine-translate your data, use an English model, and hope for the best.
Translate-train: Machine-translate the English training set to another language and fine-tune a multilingual model on that. In this case, the test set remains in the original language.
Translate-train-all: In this scenario, we machine-translate the training set to all languages and fine-tune a multilingual model on that. 

Recently \cite{Xtreme_benchmark} to incorporate a number of previously well known tasks in english in a multilingual setting. What is special about this task clinical task in a multilingual setting?

\cite{XLMR} is a state of the art multilingual model 
\cite{mt5} mT5 and demonstrate its
state-of-the-art performance on many multilingual benchmarks. 
Warum XLMR und nicht mt5? Adapter!

\cite{Ruder_embedding_survey}
While the previous methods consider a single
language at a time, multilingual representations
have recently attracted a large attention. Most
of this research focuses on ....



\cite{Ponti_typologicalLinguistics} hmmm?
\cite{madX} Adapters
\cite{xl-translations_downstream}
adapting translation to perform downstream task
\cite{zero_shot_Ponti}
Most combinations of NLP tasks and language varieties lack in-domain examples for
supervised training because of the paucity
of annotated data. How can neural models
make sample-efficient generalizations from
task–language combinations with available
data to low-resource ones?
\cite{multifit}
Cross-lingual pretrained language models
The multi-lingual BERT model is pretrained on
the Wikipedias of 104 languages using a shared
word piece vocabulary. LASER (Artetxe and
Schwenk, 2018) is trained on parallel data of
93 languages with a shared BPE vocabulary.
XLM (Lample and Conneau, 2019) additionally
pretrains BERT with parallel data. These models
enable zero-shot transfer, but achieve lower results
than monolingual models. In contrast, we focus
on making the training of monolingual language
models more efficient in a multi-lingual context.

Concurrent work (Mulcaire et al., 2019) pretrains
on English and another language, but shows that
cross-lingual pretraining only helps sometimes.

We propose Multi-lingual language
model Fine-Tuning (MultiFiT) to enable practitioners to train and fine-tune language models efficiently in their own language. In addition, we propose a zero-shot method using an existing pretrained cross-lingual model

\cite{opus_mt} off the shelf translation systems that are state of the art.
oder doch google und OPUS nicht erwaehnen. 

OpusMT und GoogleMT wurden fuer das griechische und spanische EMEA Corpus verglichen aehnliche Perfomarmance fuer beide MT in beiden Sprachen.
It was the only medical parallel corpora found that is available in both spanish and greek.
BLEU scores EMEA 

Multilingual limitations!!
Pires et. al
\cite{multiviewRegularization} 
"Multilingual pre-trained representations (Devlin
et al., 2019; Huang et al., 2019; Conneau and Lample, 2019; Conneau et al., 2020) are now an essential component of state-of-the-art methods for
cross-lingual transfer (Wu and Dredze, 2019; Pires
et al., 2019). 
These methods pretrain an encoder by
learning in an unsupervised way from raw textual
data in up to hundreds of languages which can then
be fine-tuned on annotated data of a downstream
task in a high-resource language, often English, and
transferred to another language. In order to encode
hundreds of languages with diverse vocabulary, it
is standard for such multilingual models to employ
a shared subword vocabulary jointly learned on the
1Code for the method is released here:
https://github.com/cindyxinyiwang/
multiview-subword-regularization
en excitement fr excita/tion
de Auf/re/gung pt excita/ção
%el εν/θ/ουσι/ασμός ru волн/ение
Table 1: XLM-R segmentation of “excitement” in different
languages. The English word is not segmented while the
same word in other languages is over-segmented. A better
segmentation would allow the model to match the verb stem
and derivational affix across languages.
multilingual data using heuristic word segmentation methods based on byte-pair-encoding (BPE;
Sennrich et al., 2016) or unigram language models (Kudo and Richardson, 2018) (details in §2).
However, subword-based preprocessing can lead
to sub-optimal segmentation that is inconsistent
across languages, harming cross-lingual transfer
performance, particularly on under-represented languages"
---
we want to compare the influence of the translation artefacts on the downstream task?

\cite{tokenizationUKP}
We find that while the pretraining data
size is an important factor, a designated monolingual tokenizer plays an equally important
role in the downstream performance.
Despite recent efforts to mitigate this
issue (e.g., Chung et al. (2020) propose to cluster
and merge the vocabularies of similar languages,
before defining a joint vocabulary across all languages), the multilingual LMs still struggle with
balancing their parameters across many languages.
\cite{canine}
without explicit tokenization or
vocabulary—and a pre-training strategy that
operates either directly on characters or optionally uses subwords as a soft inductive
bias
\cite{whatToShare}

 In this work, we focus on the multilingual transfer setting where training data in
multiple source languages is leveraged to further boost target language performance.

crosslingual transfer learning (CLTL) offers the possibility of learning models for a target language
using annotated data from other languages (source
languages) (Yarowsky et al., 2001). In this paper,
we concentrate on the more challenging unsupervised CLTL setting, where no target language labeled data is used for trainining. In contrast, supervised CLTL assumes the availability of annotations in the target language.

Traditionally, most research on CLTL has been
devoted to the standard bilingual transfer (BLTL)
case where training data comes from a single
source language. In practice, however, it is often the case that we have labeled data in a few
languages, and would like to be able to utilize all
of the data when transferring to other languages.

On the other hand, the multilingual transfer
setting, although less explored, has also been studied (McDonald et al., 2011; Naseem et al., 2012;
Tackstr ¨ om et al. ¨ , 2013; Hajmohammadi et al.,
2014; Zhang and Barzilay, 2015; Guo et al., 2016),
showing improved performance compared to using labeled data from one source language as in
bilingual transfer

multilingual transfer learning (MLTL), to further boost the target language performance.
One straightforward method employed in CLTL
is weight sharing, namely directly applying the
model trained on the source language to the target
after mapping both languages to a common embedding space. 

For that we use XLM-R and use Adapters.  
We are not looking into how to represent cross-lingual embeddings better but do an in-depth analysis investigating three different languages and test how the downstream task performs comparing translation and original language.

\cite{bert_cross_lingual_effectiveness}
A new release of BERT (Devlin,
2018) includes a model simultaneously pretrained on 104 languages with impressive performance for zero-shot cross-lingual transfer
on a natural language inference task. This paper explores the broader cross-lingual potential of mBERT (multilingual) as a zero-shot
language transfer model on 5 NLP tasks covering a total of 39 languages from various language families:

Additionally, we investigate the most effective strategy for utilizing mBERT in this manner, determine to what extent mBERT generalizes away from language-specific features, and
measure factors that influence cross-lingual
transfer.

\cite{translationArtifacts}
errors accumulate in the pipeline

While most NLP resources are English-specific,
there have been several recent efforts to build
multilingual benchmarks. 
The resulting multilingual
datasets are generally used for evaluation only, relying on existing English datasets for training
 Previous work has explored 3 main
approaches to that end: machine translating the
test set into English and using a monolingual English model (TRANSLATE-TEST), 
machine translating the training set into each target language 
and training the models on their respective languages (TRANSLATE-TRAIN), 
or using English data to fine-tune a multilingual model that is then transferred to the rest of languages (ZERO-SHOT).

The dataset creation and transfer procedures described above result in a mixture of original,1
human translated and machine translated data
when dealing with cross-lingual models. In fact,
the type of text a system is trained on does not
typically match the type of text it is exposed to at
test time: TRANSLATE-TEST systems are trained on
original data and evaluated on machine translated
test sets, ZERO-SHOT systems are trained on original data and evaluated on human translated test
sets, and TRANSLATE-TRAIN systems are trained on
machine translated data and evaluated on human
translated test sets

While improvements brought by machine translation have previously been attributed
to data augmentation (Singh et al., 2019), we reject this hypothesis and show that the phenomenon
is only present in translated test sets, but not in original ones.
Instead, our analysis reveals that
this behavior is caused by subtle artifacts arising
from the translation process itself.

We experiment with two models that are representative of the state-of-the-art in monolingual and
cross-lingual pre-training: (i) ROBERTA (Liu et al.,2019), which is an improved version of BERT that
uses masked language modeling to pre-train an English Transformer model, and (ii) XLM-R

when generalizing from English to the rest of languages. However, our work shows that there is
another factor that can have a much larger impact:
the loss of performance when generalizing from
original to translated data. 

However, we show that it is training on translated data,
rather than training on the target language, that is
key for this approach to outperform ZERO-SHOT as
reported by previous authors.
\cite{xlda}

Recent work on pretraining natural language processing systems (Devlin et al., 2018; Radford
et al., 2018; Howard and Ruder, 2018; Peters et al.,
2018; McCann et al., 2017) has led to improvements across a wide variety of natural language
tasks (Wang et al., 2018; Rajpurkar et al., 2016;
Socher et al., 2013; Conneau et al., 2018).

One of the most common ways to leverage multilingual data is to use transfer learning. Word
embeddings such as Word2Vec (Mikolov et al.,
2013b) or GloVe (Pennington et al., 2014) use
large amounts of unsupervised data to create
task-agnostic word embeddings which have been
shown to greatly improve downstream task performance. Multilingual variants of such embeddings (Bojanowski et al., 2017) have also shown
to be useful at improving performance on common tasks across several languages. More recently
contextualized embeddings such as CoVe,
ElMo, ULMFit and GPT (McCann et al., 2017;
Peters et al., 2018; Howard and Ruder, 2018; Radford et al., 2018) have been shown to significantly
improve upon aforementioned static embeddings.



XLDA can
be used with both pretrained and randomly initialized models without needing to explicitly further
align the embeddings. To apply XLDA to any natural language input, we simply take a portion of
that input and replace it with its translation in another language. This makes XLDA perfectly compatible with recent methods for pretraining (Lample and Conneau, 2019; Devlin et al., 2018). Additionally, the approach seamlessly scales for many
languages and improves performance on all highand low-resource languages tested including English, French, Spanish, German, Greek, Bulgarian, Russian, Turkish, Arabic, Viet



\cite{use_machine_translation}

\cite{zeroToHero}
\cite{subectivity_analysis_mt}
\cite{syntactic_transfer_bilingual_lexicon}

\cite{coding_book}
\cite{bert_medical_code_assignement}

\cite{brasilian_biobert}
Other attempts have been made to implement code prediction in other languages than English






\paragraph{multilingual models and translation in clinical domain}

clinical text in Spanish but used only translation and incorporated mimic \cite{clef_SchaferF20}


